Soliton Propagation in Chains with Simple Nonlocal Defects

We study the propagation of solitons on complex chains built by inserting finite graphs at two sites of an unbranched chain. We compare numerical findings with the results of an analytical linear approximation scheme describing the interaction of large-fast solitons with non-local topological defects on a chain. We show that the transmission properties of the solitons strongly depend on the structure of the inserted graph, giving a tool to control the soliton propagation through the choice of pertinent graphs to be attached to the chain.

==> readme <==
%
% ------------------------------------------------------------------- %
%   This file is the main README file for the REVTeX v3.0 macro set   %
%                     version 3.0, November 10 1992                   %
% ------------------------------------------------------------------- %
%
% IMPORTANT NOTICE: You are not allowed to change this readme file.
%

Copyright (c) 1992 by American Physical Society, American Institute of
                   Physics, Optical Society of America.  All rights reserved.

Other files in this package are copyrighted as stated, and their rights
are reserved by their respective owners.

This version of REVTeX is a cooperative product of the American Physical
Society (APS), American Institute of Physics (AIP), and Optical Society of
America (OSA).

The Joint Society Task Force, comprised of AIP and AIP Member Societies has
appointed a REVTeX Working Group in order to coordinate the development and
evolution of a joint electronic publishing product and mark-up language
standards amongst the participating societies.

Those authors interested in publishing articles in the journals of the
American Astronomical Society should use AASTeX (the LaTeX-based mark-up
developed by the American Astronomical Society). One of the primary objectives
of the REVTeX Working Group is to make REVTeX and AASTeX as similar as
possible. Authors will use many of the same mark-up tags in manuscripts prepared
using either REVTeX or AASTeX. Style differences in the journals---for example,
the manner in which citations are handled (numerical reference or author/date
format)---require that authors actually write different text. Thus, it is
important that authors identify the journal they intend to publish in and use
the appropriate electronic publishing product.


%%%%%%%%%%%%%%%%%%%%%%% RESTRICTIONS ON USE %%%%%%%%%%%%%%%%%%%%%%%

Files in this package may only be distributed or changed according
to the following restrictions.


Distribution of unchanged versions:

  You are NOT ALLOWED to take money for the distribution or use of
  these files except for a nominal charge for copying, etc.

  Redistribution of unchanged files is allowed provided that all files
  listed in this readme file are distributed together.

  If you receive only some of these files from someone, complain!


Generation and distribution of changed versions:

  The generation of changed versions of the files included in the
  packages is allowed under the following restrictions:

  - Rename the file before you make any changes to it.

  - Acknowledge the origin of the changed version in the file and
    keep the information that it (or a changed version) has to be
    distributed under the restrictions mentioned in this file.

  - Change any ERROR REPORT address so that we don't get error
    reports for files *not* maintained by us.


The distribution of changed versions of the files included in the
package is allowed under the following restrictions:

  - Provide the user with information how to obtain the original
    package or, even better, distribute it with your files.

  - Make sure that the changed versions contain a notice that
    prevents others from taking money for distribution or use of your
    files, i.e., they have to be distributed under the restrictions
    mentioned in this file.


%%%%%%%%%%%%%%%%%%%%%%% REVTeX DISTRIBUTION %%%%%%%%%%%%%%%%%%%%%%%

Files in the complete REVTeX 3.0 distribution:

  (a) the general files:
      README           % this file
      revtex.sty       % main style file
      manintro.tex     % introduction for input guide
      manend.tex       % appendixes for input guide
  (b) AIP-specific files
      manaip.tex       % AIP chapter for input guide
  (c) APS-specific files
      aps.sty          % main society-specific style file for APS macros
      aps10.sty        % internally called style for galley-format output
      aps12.sty        % internally called style for preprint-format output
      apssamp.tex      % sample file
      manaps.tex       % APS chapter for input guide
      prabib.sty       % internally called style for normal-style citations
      prbbib.sty       % internally called style for PRB-style citations
      prsty.bst        % Physical Review--style BibTeX style file
      reftest.tex      % Citation and bibliography analyzer
      template.aps     % template file; copy to filename.tex and edit that file
      version2.sty     % style file for running v2.x REVTeX files in v3.0
  (d) OSA-specific files
      osa.sty          % Society-specific style file for OSA journals
      osa10.sty        % Fonts and format style file for OSA journals
      osa12.sty        % Fonts and format style file for OSA journals
      osabib.sty       % Society file for bibliography style
      template.tex     % OSA template for creating a manuscript
      sample.tex       % a longer sample of REVTeX use
      manosa.tex       % OSA chapter for input guide
      josaa.tex        % sample JOSA A paper
      josab.tex        % sample JOSA B paper
      aplop.tex        % sample Applied Optics paper


%%%%%%%%%%%%%%%%%%%%%%% GETTING STARTED %%%%%%%%%%%%%%%%%%%%%%%

You must have TeX and LaTeX running to use these macros. All macros
run on a standard LaTeX format.

Installing to just test the macros can be accomplished by copying all the
files into an unused directory, then changing to that directory. All the
files and facilities of REVTeX should then be usable while you are in that
directory.

A more permanent installation would usually mean installing the .sty files
and reftest.tex file into the directory where TeX usually looks for input
files, the .bst files into the directory where BibTeX usually looks for its
style files, and the rest of the files into a REVTeX working directory or a
public directory, depending on your system setup. Care should be taken to
avoid writing over files already present. The files in the REVTeX package have
been named to help avoid this problem, but there can be no guarantee that
our file names are unique.

If you are permanently upgrading an older version of REVTeX (<3.0), the files
from the old version should be removed first. You may delete these files or
save them somewhere where they will not be found by TeX when it looks for
style files. Here is a list of the older files:

      readme        % make sure you only delete the REVTeX readme!
      revtex.sty
      aps.sty
      aps10.sty
      aps12.sty
      preprint.sty
      eqsecnum.sty
      smplea.tex
      smpleb.tex
      smplec.tex
      apguide.tex

Older versions of REVTeX (<3.0) will not coexist with this version.

The next thing you need to do is run LaTeX on the files for the input guide.
The input guide consists of common introductory material (manintro.tex),
society-specific chapters (manaps.tex for APS, manosa.tex for OSA, and
manaip.tex for AIP), and common appendixes (manend.tex). Run LaTeX on, and
print, manintro.tex, the desired society-specific chapters, and manend.tex.
Gathering the printed material together in order will provide all needed
information. There is a general table of contents in manintro.tex, and
separate tables of contents in each society's chapter. Carefully read the
intructions in the appropriate chapter of the Input Guide. The sample file(s)
and template will also contain useful examples and explanations.

You may get a number of "Underfull \hbox . . ." messages when running the
documentation and samples; these are normal. Also, you may need to LaTeX
these files three times to complete all references and build the table of
contents.

If needed, consult a local (La)TeX user or system support person for
information on how to run LaTeX and print its output on your local system.


%%%%%%%%%%%%%%%%%%%%%%% ERROR REPORTS %%%%%%%%%%%%%%%%%%%%%%%

Before you report an error please check that

  - the error isn't caused by obsolete versions of other software.
    LaTeX from 1986 is a good candidate; for example, negative indents
    (outdents) following an equation environment.

  - you use an original version of the package.


If you think you have found a genuine bug please report it, together
with the following information:

  - version of the REVTeX file(s)

  - version (date!) of your LaTeX

  - a short test file showing the behavior with all unnecessary
    coding removed. The log file showing the problem might also help.


Errors should be reported to the person listed in your copy of the
user guide.



